Towards Calibrated Robust Fine-Tuning of Vision-Language Models

Improving out-of-distribution (OOD) generalization during in-distribution (ID) adaptation is a primary goal of robust fine-tuning of zero-shot models beyond naive fine-tuning. However, despite decent OOD generalization performance from recent robust fine-tuning methods, confidence calibration for reliable model output has not been fully addressed. This work proposes a robust fine-tuning method that improves both OOD accuracy and confidence calibration simultaneously in vision language models. Firstly, we show that both OOD classification and OOD calibration errors have a shared upper bound consisting of two terms of ID data: 1) ID calibration error and 2) the smallest singular value of the ID input covariance matrix. Based on this insight, we design a novel framework that conducts fine-tuning with a constrained multimodal contrastive loss enforcing a larger smallest singular value, which is further guided by the self-distillation of a moving-averaged model to achieve calibrated prediction as well. Starting from empirical evidence supporting our theoretical statements, we provide extensive experimental results on ImageNet distribution shift benchmarks that demonstrate the effectiveness of our theorem and its practical implementation.

==> thm.tex <==
\section{Theoretical Analysis on OOD Generalization and Calibration}
\label{sec:theoritical_analysis}
We first identify the factors that affect OOD generalization and calibration errors under circumstances where only ID data is accessible.
We take inspiration from the generalization bound of domain adaptation literature~\cite{bendavid2010, NEURIPS2018_717d8b3d} while remarkably adapting the analysis to consider both OOD classification and calibration error at the same time in a more practical way.

Let $\mathcal{D}$ be a domain on input space $\mathcal{X}$ and $\mathcal{Y}=\{0,1\}$ be a label space for a binary classification. Among the hypothesis function $h:\mathcal{X}\rightarrow[0,1]$, we define $h_{0}(\cdot)$ as a desired calibrated predictor for label $y$, which minimizes the calibration error $\mathbb{E}_{ x \sim \mathcal{D}}[(h(x) - c(x))^{2}]$ \cite{murphy1972}, where $c(x) = \mathbb{E}_{y}[y|h(x)]$ is the expected value of $y$ given a prediction $h(x)$. That is, $h_{0}$ always produces the calibrated prediction for $y$ given $x$ so that the output confidence $h_{0}(x)$ matches the expectation of $y$ over the subset of samples that have the same confidence as $h_{0}(x)$. Our goal is to learn a hypothesis function $h(\cdot)$ that outputs reliable probability on samples from the unseen OOD domain, which is defined by a distribution $\mathcal{D}_{\text{OOD}}$, as well as on the ID domain $\mathcal{D}_{\text{ID}}$, where the predictor is trained on. In essence, the error $\varepsilon_{\mathcal{D}}(h)=\mathbb{E}_{x \sim \mathcal{D}}[(h(x) - h_{0}(x))^{2}]$ should be small for two different domains $\mathcal{D} \in \{\mathcal{D}_{\text{ID}}, \mathcal{D}_{\text{OOD}}\}$. In this work, we concentrate on the covariate shift scenario (\S\ref{sec:preliminary_background}) that only the marginal distribution over $\mathcal{X}$ changes while the distribution over $\mathcal{Y}$ is preserved.

Let the optimal hypothesis $h^{*}$, which minimizes a combination of errors on both ID and OOD domain, be $h^{*}:= \argminA_{h \in \mathcal{H}} \varepsilon_{\mathcal{D}_{\text{ID}}}(h)+\varepsilon_{\mathcal{D}_{\text{OOD}}}(h)$, and $\Delta$ denote the optimal joint error $\Delta:= \varepsilon_{\mathcal{D}_{\text{ID}}}(h^{*})+\varepsilon_{\mathcal{D}_{\text{OOD}}}(h^{*})$. We derive our novel bounds for the OOD calibration error and OOD classification error. 
\begin{theorem}
Let $h:\mathcal{X}\rightarrow[0,1]$ be a real-valued function which has structure $h(x)=\sum_{i=1}^{d}h_{i}(x_{i})$ where $h_{i}$ is an arbitrary one-dimensional function, and $h(\cdot)$ is in a hypothesis class $\mathcal{H}$ that has pseudo dimension $\mathcal{P} dim(\mathcal{H})=d_{h}$, $\hat{\mathcal{D}}_\text{ID}$ be an $N$-size empirical distribution on $\text{ID}$ domain. If $(x_{i},x_{j})$ is a bi-variate Gaussian random variable for every $i,j \in [d]$, then for any $\delta \in (0,1)$ and for all $h$, the following bounds hold with probability at least $1-\delta$:
\makeatother
{
\small
% \footnotesize
\begin{flalign}
\text{i}) \ \
 &\varepsilon_{\mathcal{D}_{\text{OOD}}}(h) \le \varepsilon_{\hat{\mathcal{D}}_{\text{ID}}}(h) + {\frac{d}{\sigma_{\text{min}}(\tilde{\Sigma}_{\mathcal{D}_{\text{ID}}})}} + \Delta + \mathcal{O} \left(\sqrt{{1 \over N} \log {{({N \over d_{h}})}^{d_{h}}({1 \over \delta})} }\right),&  \label{eq:cal_bound}\\
\text{ii}) \ \
&\mathbb{E}_{\mathcal{D}_{\text{OOD}}}[(h(x)-y)^{2}] + \mathbb{E}_{\mathcal{D}_{\text{OOD}}}[c(x)^{2}] -1 \le \varepsilon_{\hat{\mathcal{D}}_{\text{ID}}}(h) + {\frac{d}{\sigma_{\text{min}}(\tilde{\Sigma}_{\mathcal{D}_{\text{ID}}})}} + \Delta + \mathcal{O} \left(\sqrt{{1 \over N} \log {{({N \over d_{h}})}^{d_{h}}({1 \over \delta})} }\right),& \label{eq:cls_bound}
 \end{flalign}
}
\end{theorem} \label{thm:bound_new2}
where $\tilde{\Sigma}_{\mathcal{D}_{\text{ID}}}{:=}\mathbb{E}_{\mathcal{D}_{\text{ID}}}[\tilde{x}\tilde{x}^{T}]$ is a covariance matrix of $d$-dimensional normalized input $\tilde{x}=(\tilde{x}_{1},...,\tilde{x}_{d})$, where $\tilde{x}_{i}{:=}(x_{i} - \mathbb{E}[x_{i}]) \text{Var}(x_{i})^{-1/2}$ and $\sigma_{\text{min}}(M)$ is the smallest singular value of a matrix $M \in \mathbb{R}^{d_{1}\times d_{2}}$. These theoretical results can be directly applied to the intermediate representation of a neural network by setting the input variable $x$ as a representation vector~\cite{NIPS2006_b1b0432c, zhao2019learning}, so we will assume the input as an image representation of the visual encoder in following sections. Note that 1) the LHS of the first inequality (eq.\eqref{eq:cal_bound}) indicates \textbf{OOD calibration error}, 2) two terms in the LHS of the second inequality (eq.\eqref{eq:cls_bound}) denote \textbf{OOD classification error} in terms of $L_{2}$ loss and prediction sharpness in OOD domain, and 3) both inequalities have the same RHS, which contains the empirical estimate of \textbf{ID calibration error}, the reciprocal of the \textbf{smallest singular value of ID input covariance matrix}, and remaining irreducible terms that depend on the problem setup.

Based on our analysis, we expect the potential of reducing the upper bound of OOD calibration error and the sum of OOD classification error and prediction sharpness by minimizing the first two terms of RHS in both bounds: the empirical ID calibration error and the reciprocal of minimum singular value of the normalized ID covariance matrix. In \S\ref{sec:method}, we devise a realization of this theoretical concept.
